Learning Energy Decompositions for Partial Inference of GFlowNets

This paper studies generative flow networks (GFlowNets) to sample objects from the Boltzmann energy distribution via a sequence of actions. In particular, we focus on improving GFlowNet with partial inference: training flow functions with the evaluation of the intermediate states or transitions. To this end, the recently developed forward-looking GFlowNet reparameterizes the flow functions based on evaluating the energy of intermediate states. However, such an evaluation of intermediate energies may (i) be too expensive or impossible to evaluate and (ii) even provide misleading training signals under large energy fluctuations along the sequence of actions. To resolve this issue, we propose learning energy decompositions for GFlowNets (LED-GFN). Our main idea is to (i) decompose the energy of an object into learnable potential functions defined on state transitions and (ii) reparameterize the flow functions using the potential functions. In particular, to produce informative local credits, we propose to regularize the potential to change smoothly over the sequence of actions. It is also noteworthy that training GFlowNet with our learned potential can preserve the optimal policy. We empirically verify the superiority of LED-GFN in five problems including the generation of unstructured and maximum independent sets, molecular graphs, and RNA sequences.

==> 4_related.tex <==
\section{Related works}
\label{sec:related}

\textbf{Model-based GFlowNet.} 

\textbf{Generative augmented flow network.} 

\textbf{Reward redistribution.} Yet, such ideas have not been explored with GFlowNets

==> 5_experiments.tex <==
\section{Experiment}
\label{sec:experiment}

We extensively evaluate our algorithm on various domain, including set and bag generation \citep{pan2023better,towardsunderstandinggflownets}, molecular generation \citep{bengio2021flow}, RNA sequence generation \citep{jain2022biological}, and maximum independent set \citep{zhang2023let}. Following prior studies \citep{bengio2021gflownet,malkin2022trajectory,pan2023better}, we consider the number of modes and the average tok-$k$ score as base metrics, which are measured via samples collected during training.\footnote{We also evaluate how well generative distribution match the target energy distribution in \Cref{subsec:ablation}.} For all experiments, we report the performance measured with three different random seeds. 


\input{resources/fig_set_only}

\input{resources/fig_bag}


\subsection{Set generation} \label{subsec:experiment_bag}

We first validate our method on two types of set generation tasks, set \citep{pan2023better} and bag \citep{towardsunderstandinggflownets} generations. The action of both tasks is adding entities to the current set. However, their energy evaluations differ; both are defined as follows:
\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.0mm]
\item \textbf{Set}: The energy is evaluated by accumulation of individual entity energies, so the intermediate energy gain has complete information to identify contribution of individual action.
\item \textbf{Bag}: The energy is evaluated by inclusion of seven or more repeated same entity, so the intermediate energy is less informative to identify contribution of individual action, akin to \Cref{toy:toytoy}.
\end{itemize}
We compare our method with GFlowNet and FL-GFN, where both of them are implemented with DB and subTB. The detailed settings are described in \Cref{appx:exp_setup}.

\textbf{Results. } The results for set and beg generations are presented in \Cref{fig:set} and \Cref{fig:bag}, respectively. In \Cref{fig:set}, one can see that our method shows similar performance compared to FL-GFN on DB and subTB. Although intermediate energy provides complete information, our method can achieve similar performance without energy evaluation for intermediate states. In \Cref{fig:bag}, one can see that our method excels on bag generation. These results stem from the superiority of learning-based approach over limitations in energy-based partial inference, i.e., sparse local credit signal.



\subsection{Molecule generation}

\input{resources/fig_graph}

Next, we validate LED-GFN on molecule generation task \citep{bengio2021flow}, which aims to find molecules with low binding energy to the soluble epoxide hydrolase protein. In this tasks, a molecule is generated by constructing a junction trees \citep{jin2018junction}, where the action is adding a molecular building blocks. The binding energy is computed by a pre-trained oracle \citep{bengio2021flow}. 

In this experiment, we consider the baselines PPO \citep{schulman2017proximal}, and three GFN with DB, TB \citep{malkin2022trajectory}, subTB. We also compare with GAFN, \citep{pan2023generative} and FL-GFN. Both are implemented on subTB. The overall implementations and experimental settings follow prior studies \citep{bengio2021flow,pan2023better}, which are described in \Cref{appx:exp_setup}.

\textbf{Results. } The results are presented in \Cref{fig:molecule}. One can see that LED-GFN outperforms considered baselines in enhancing the average reward of unique top-$100$ molecules and the number of modes found. These results highlight that LED-GFN also benefits to improve creidit assignment for real-world generation problems which have large state spaces.

\subsection{RNA sequence generation}

\input{resources/fig_protein}

We also consider another practical generation task for discovering diverse and promising RNA sequences that bind to human transcription factors \citep{barrera2016survey,trabucco2022design,jain2022biological}. The action is appending or prepending the amino acid in current sequences. The energy is computed by wet-lab measured DNA binding activity to a Sine Oculis Homeobox Homolog 6 \citep{barrera2016survey}. We consider the same baselines as in molecule generation task. 

\textbf{Results. } The results are presented in \Cref{fig:protein}. One can see that LED-GFN outperforms considered baselines. Furthermore, FL-GFN only makes minor differences compared to GFN, while LED-GFN makes noticeable improvements. These results highlight that energy-based partial inference may not enhance performance in practical domain, while the learning-based approach make improvements.


%\footnote{In \Cref{fig:relative}, we also highlight the superiority of LED-GFN for approximating the target distribution.}  


\subsection{Maximum independent set}

In solving maximum independent set, we further show that LED-GFN can achieve similar performance compared to FL-GFN, \textit{even though the intermediate energy is ideal for providing informative signal to identify the contribution of action} \citep{zhang2023let}. 

\input{resources/fig_comb}

Here, we compare performance on validation graphs following \citet{zhang2023let}. At each step, we sample $50$ solutions for each validation graph to measure the average scores and the number of modes (greater than $18.5$). The overall implementations and hyper-parameters follow prior studies \citep{zhang2023let}.

\textbf{Results. } As illustrated in \Cref{fig:combinatorial}, one can see that our approach achieves similar performance to FL-GFN, even though the intermediate state energy is carefully designed with domain knowledge. These results highlight that the potentials of LED-GFN can be informative as much as ideal local credit which provides complete identification of the action contributions.




\subsection{Ablation studies} \label{subsec:ablation}

\input{resources/fig_approximation}

\input{resources/fig_compare_method}

\textbf{Goodness-of-fit to the true Boltzmann distribution.} We also show that how well our algorithm make good sampling distribution to match the target distribution, i.e., Boltzmann distribution. We measure the relative mean error between the empirical generative distribution and target distribution following \citet{towardsunderstandinggflownets}. In \cref{subfig:relative_bag,subfig:relative_rna}, one can observe that LED-GFN achieves better approximation to target distribution compared to considered baselines.

\textbf{Diversity vs. high score.} Next, we further verify that our algorithm not only generates high score samples but also diverse molecules. Specifically, we analyze the trade-off between average score of top-$100$ samples and diversity of top-$100$ samples. To measure diversity, we compute the average pairwise Tanimoto similarity \citep{bajusz2015tanimoto}. In \Cref{subfig:simil_mol}, we plot the Tanimoto similarities with respect to the average of top-$100$ molecules. Here, one can see that LED-GFN achieves better diversity with respect to the average scores.  

\textbf{Energy decomposition learning vs. alternative potential learning.} We further investigate various potential function learning schemes, 
\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.0mm]
\item One may train a proxy model $\phi_{\theta}:\mathcal{X}\rightarrow \mathbb{R}$ to predict the terminal energy, and utilize it to compute potentials $\phi_{\theta}(s\rightarrow s')=\phi_{\theta}(s')-\phi_{\theta}(s)$. This approach can be interpreted as extension of model-based GFlowNet \citep{jain2022biological} for partial inference.
\item One can consider a LSTM which takes trajectory $(s_0,a_0,\cdots,s_{n-1},a_{n-1})$ to predict the object energy $\mathcal{E}(x)$. Then, the potential $\phi_{\theta}(s_t\rightarrow s_{t+1})$ can be designed as the difference between two subsequent predictions on $(s_0,a_0,\cdots,s_{t},a_{t})$ and $(s_0,a_0,\cdots,s_{t+1},a_{t+1})$, akin to LSTM-based reward redistribution methods in reinforcement learning \citep{arjona2019rudder}.
\end{itemize}

In \Cref{fig:method_compare}, we compare each method in molecule and set generation tasks, where each of them is implemented on subTB-based objective. Here, one can see that least square-based approach shows most competitive performance due to its capabilities to produce dense and informative potentials. 

\input{resources/fig_reducing_variance}

\textbf{Variance-constrained vs. unconstrained potentials.} We also analyze how reducing variance of potentials benefits. To this end, we compare the energy decomposition learning with regularization and one without regularization for reducing the variance, i.e., we set $\lambda=1$ in \Cref{eq:least_square}. In \Cref{fig:regularization}, one can see that applying regularization shows more promising performance. These results highlight that inducing dense local credits signal plays a significant role in improving performance.

%\input{resources/fig_analysis_predicted}

\textbf{Number of energy evaluation vs. performance} We also analyze the performance over the number of energy evaluation, which can be expensive. In \Cref{fig:oracle_calls}, one can see that FL-GFN can not improve performance since it should evaluate the energy for all every visited intermediate states, whereas LED-GFN uses a potential function without energy evaluation for intermediate states.



%\textbf{Analysis on potentials.} We also analyze how potential function evaluates local credit. In \Cref{fig:first_fig}, one can see that LED-GFN produces informative local credit. We further analyze the 


==> resources/fig_analysis_predicted.tex <==
\begin{figure}[t]
\centering
\hfill
\begin{subfigure}[t]{0.22\linewidth}
\centering
  \includegraphics[width=\linewidth]{example-image}
  \caption{Set generation}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.22\linewidth}
\centering
  \includegraphics[width=\linewidth]{example-image}
  \caption{Set generation}
\end{subfigure}
\hfill
\caption{
}\label{fig:analysis}
\vspace{-.1in}
\end{figure}


==> resources/fig_comb.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
    \includegraphics[width=0.95\linewidth]{resources/figures/paper_GFlow-MIS_inter.pdf}
    \caption{\textbf{The performance on maximum independent set.} The LED-GFN achieve similar performance to the FL-GFN with a ideal energy function based on domain knowledge.}\label{fig:combinatorial}
\end{wrapfigure}

==> resources/tab_molecule.tex <==
\begin{wrapfigure}{r}{0.43\textwidth}
\centering
    %\setlength{\belowcaptionskip}{-22pt}
    \vspace{.05in}
    \begin{subfigure}[t]{0.49\linewidth}
    \centering
        \includegraphics[width=\linewidth]{nips/resources/figures/synthetic_true.pdf}
        \caption{Scattered}\label{subfig:first_synthetic}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\linewidth}
    \centering
        \includegraphics[width=\linewidth]{nips/resources/figures/synthetic_true_type2.pdf}
        \caption{Localized}\label{subfig:second_synthetic}
    \end{subfigure}
    \caption{Illustration of two scenarios. \sethlcolor{OliveGreen}\hl{Green} highlights known labels.}\label{fig:synthetic_scenario}
\vspace{0.3in}
\centering
\captionof{table}{The transductive node classification accuracy on synthetic data. \textbf{Bold} numbers indicate the best performance.
}\label{tab:transductive_synthetic}
\scalebox{0.83}{
\begin{tabular}{lcc}
\toprule
Method & Scattered & Localized \\
\midrule
GCN \citep{kipf2016semi} & {50.1}\stdv{0.6} & {51.3}\stdv{1.4} \\
$+$ GMNN \citep{qu2019gmnn} & {64.2}\stdv{3.2} & {48.2}\stdv{4.8} \\
$+$ G$^{3}$NN \citep{ma2019flexible} & {50.1}\stdv{0.6} & {51.3}\stdv{1.4} \\
$+$ CLGNN \citep{hang2021collective} & {87.0}\stdv{2.4} &  {53.4}\stdv{2.1}\\
$+$ DPM-SNC (ours) & \textbf{98.5}\stdv{0.7} & \textbf{90.9}\stdv{3.4}  \\
\bottomrule
\end{tabular}
}
\end{wrapfigure}
